Regret Minimization for Piecewise Linear Rewards: Contracts, Auctions, and Beyond

Most microeconomic models of interest involve optimizing a piecewise linear function. These include contract design in hidden-action principal-agent problems, selling an item in posted-price auctions, and bidding in first-price auctions. When the relevant model parameters are unknown and determined by some (unknown) probability distributions, the problem becomes learning how to optimize an unknown and stochastic piecewise linear reward function. Such a problem is usually framed within an online learning framework, where the decision-maker (learner) seeks to minimize the regret of not knowing an optimal decision in hindsight. This paper introduces a general online learning framework that offers a unified approach to tackle regret minimization for piecewise linear rewards, under a suitable monotonicity assumption commonly satisfied by microeconomic models. We design a learning algorithm that attains a regret of $\widetilde{O}(\sqrt{nT})$, where $n$ is the number of ``pieces'' of the reward function and $T$ is the number of rounds. This result is tight when $n$ is \emph{small} relative to $T$, specifically when $n \leq T^{1/3}$. Our algorithm solves two open problems in the literature on learning in microeconomic settings. First, it shows that the $\widetilde{O}(T^{2/3})$ regret bound obtained by Zhu et al. [Zhu+23] for learning optimal linear contracts in hidden-action principal-agent problems is not tight when the number of agent's actions is small relative to $T$. Second, our algorithm demonstrates that, in the problem of learning to set prices in posted-price auctions, it is possible to attain suitable (and desirable) instance-independent regret bounds, addressing an open problem posed by Cesa-Bianchi et al. [CBCP19].

==> instance_dep.tex <==
\section{An instance-dependent bound }\label{sec:InstanceDep}


In this section, we show that the regret guarantees attained by Algorithm~\ref{alg:main} can be improved when the learner has access to an instance-parameter parameter related to the smallest jump gap.
% 
%Specifically, we show that with a suitable modification of Algorithm~\ref{alg:main}—that exploits a suitable information about the instance—it is possible to reduce the regret suffered by Algorithm~\ref{alg:main}.
%
A similar instance-dependent analysis is performed in~\cite{cesa2019dynamic} in the context of posted-price auctions.
%
Specifically, \citet{cesa2019dynamic} show that when the learner has prior knowledge of a lower bound $\gamma > 0$ on the probability of the buyer selecting any valuation, it is possible to design an algorithm whose regret guarantees satisfy:
%
$$R_T\le\mathcal{O}\left( \frac{n\log(T)\log\log(T)}{\gamma^2} + \sum_{i\in[n]:d_i>0}\frac{\log(T)}{d_i}\right),$$
%
where the parameters $d_i$ encode suboptimality gaps with respect to an optimal price. %\albo{non capisco}
%
In BwMJ problems, an equivalent instance-specific parameter is the smallest jump gap $\gamma \coloneqq \min_{i \in [n-1]}{\mu_{i+1} - \mu_{i}}$.
%
%Thus, the parameter $\gamma>0$ encodes the minimum \emph{gap} between two consecutive jumps. 
%
In the following, we propose an algorithm that works for the general framework of BwMJ—and thus for posted-price auctions—and improves the regret guarantees in~\cite{cesa2019dynamic}.


Two observations are in order. First, an instance-dependent logarithmic upper bound cannot be achieved without knowledge of $\gamma$.
%
Intuitively, it is not possible to decide whether to stop looking for smaller jumps or not. 
%
A similar result is proved by~\citet{cesa2019dynamic}, who show that it is impossible to achieve $\widetilde{\mathcal{O}}(\sqrt{T})$ regret in the worst case, \emph{i.e.}, when $\gamma \simeq\nicefrac{1}{\sqrt{T}}$, and logarithmic regret when $\gamma$ is constant.
%
Second, our algorithm improves the regret guarantees in~\citep{cesa2019dynamic} by a factor proportional to $\nicefrac{1}{\gamma}$ (see \Cref{thm:MainThmDep}).
%
\begin{comment}
\hrule
achieved in [Cesa-Bianchi et al ., 2019] for
posted-price auction settings. Indeed, in such a scenario, Cesa-Bianchi et al . [2019] provide an
algorithm whose regret guarantees satisfy:


In this section we show that is it pobbile to achieve an inst-dep boun mdofying algo 1 in order tot employ an inforamtio related to the instance.
%
Look, the same proble was studied was tudied by cseabianche in posted-price auctions
%
Cesa assume that the learner has access to a parameter $\gamma>0$ defining the minimum gap between two buyer's valuations.\footnote{\bac{definre $d_i$} } 
%
This is equivalent to assuming, within the BwMJ framework, that the learner has access to a parameter $\gamma\coloneqq \min_{i\in[n-1]}\{\mu_{i+1}-\mu_{i}\}$ encoding the minimum \emph{gap} between two consecutive jumps.  
%
We conclude the paper by showing that with a slight modification to Algorithm~\ref{alg:main}, it is possible to improve the instance-dependent regret guarantees achieved in~\cite{cesa2019dynamic} for posted-price auction settings.  
%
Indeed, in such a scenario, \citet{cesa2019dynamic} provide an algorithm whose regret guarantees satisfy:
%
$$R_T\le\mathcal{O}\left( \frac{n\log(T)\log\log(T)}{\gamma^2} + \sum_{i=1}^{n}\frac{\log(T)}{d_i}\right),$$
%
when the learner has access to a parameter $\gamma>0$ defining the minimum gap between two buyer's valuations.\footnote{\bac{definre $d_i$} } 
%
This is equivalent to assuming, within the BwMJ framework, that the learner has access to a parameter $\gamma\coloneqq \min_{i\in[n-1]}\{\mu_{i+1}-\mu_{i}\}$ encoding the minimum \emph{gap} between two consecutive jumps.  
%
In the following, we prove that under the assumption that the learner has access to such a parameter $\gamma > 0$, it is possible to achieve better regret guarantees than those of~\citet{cesa2019dynamic} for the general BwMJ framework.
\hrule
\end{comment}

Algorithm~\ref{alg:instance_dep} follows the same steps as Algorithm~\ref{alg:main} for all epochs $j \in \mathbb{N}_{+}$ in which the condition $\Delta_j\coloneqq\nicefrac{1}{2^j}\ge \nicefrac{\gamma}{4}$ is satisfied.
%
The only difference from Algorithm~\ref{alg:find_bp} is that, whenever the \texttt{Find-Jumps} procedure identifies a sufficiently small interval containing a jump discontinuity, it stores such interval in the set $\mathcal{J}$.
%
We refer the reader to Appendix~\ref{sec:AppendixDep} for the pseudocode of this modified \texttt{Find-Jumps} procedure.
%
When the condition $\Delta_j \ge \nicefrac{\gamma}{4}$ no longer holds, Algorithm~\ref{alg:instance_dep} iterates over the intervals within $\mathcal{J}$ and adds the right extreme of each $J \in \mathcal{J}$ to the set $\mathcal{W}$.
%
Finally, Algorithm~\ref{alg:instance_dep} runs the UCB1~\cite{Cesa2002Finite} algorithm, using $\mathcal{W}$ as its set of arms.
%
%
%
%
\begin{algorithm}[!htp]
	\caption{\texttt{Instance-Dependent RJI-OS} {(\texttt{ID-RJI-OS}})}
	\label{alg:instance_dep}
	\begin{algorithmic}[1]
		\Require Number of rounds $T \in \mathbb{N}_+$, parameter $\gamma>0$
		\State Set $\mathcal{I}_1 \gets \{ [0,1] \}$, $ \mathcal{T}_{1}\gets  \varnothing $, $\mathcal{J}\gets \varnothing $, $ \mathcal{W}\gets \{ 0 \}$
		\For{ $j \in \mathbb{N}_{+}$} 
		\State	$\Delta_j \gets \nicefrac{1}{2^{j}}$
		\If{$\Delta_j\ge \gamma/4$ }
		\State Execute Lines~\ref{line:endformain}-\ref{line:end_first_algo} in Algorithm~\ref{alg:main} with modified \texttt{Find-Jumps}
		\Else
		%		\State $H=-\infty$ and $\mathcal{W}=\varnothing$
		\For{ $J\coloneqq[\alpha_1,\alpha_2] \in \mathcal{J}$} \label{lin:forLoopDep}
		\State $\mathcal{W}=\mathcal{W}\cup \{\alpha_2\}$
		\EndFor
		\State Run UCB1 on the set $\mathcal{W}$ \label{line:ucb1}
		\EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}

Then, the regret sufferer by Algorithm~\ref{alg:instance_dep} can be upper bounded as follows.
%
\begin{restatable}{theorem}{InstanceDep}\label{thm:MainThmDep}
	The regret suffered by Algorithm~\ref{alg:instance_dep} is bounded by $$R_T\le\mathcal{O}\left( \frac{n\log(T)\log\log(T) \log\left(\nicefrac{1}{\gamma}\right) }{\gamma} + \sum_{i\in[n]:d_i>0}\frac{\log(T)}{d_i}\right),$$
    where $d_i\coloneqq u(\alpha^\star)- u(\overline \alpha_i)$.
\end{restatable}
%
The analysis of the regret incurred by Algorithm~\ref{alg:instance_dep} relies on the learner having access to the minimum jump gap $\gamma > 0$. 
%
Thus, when the parameter $\Delta_j$ is sufficiently smaller than $\gamma$, it is possible to identify small intervals that contain the jump discontinuities. 
%
Then, by running a no-regret algorithm using the right extreme of these intervals, it is possible to achieve the desired regret guarantees.
%We observe that Theorem~\ref{thm:MainThmDep} improves the regret guarantees in~\cite{cesa2019dynamic} by a factor proportional to $\nicefrac{1}{\gamma}$ (up to logarithmic factors).
%

%
% \begin{restatable}{lemma}{...}
% 	Under the event $\mathcal{E}$, if $\textnormal{UCB-1}$ is executed as a sub-procedure of  Algorithm~\ref{alg:instance_dep}, then there exists an $\alpha_2 \in \mathcal{W}$ such that $u(\alpha_2) \ge \textnormal{OPT}-\nicefrac{1}{T}$.
% \end{restatable}
% \begin{proof}
% %	
% %
% %
% %We first show that, for each epoch $j \in \mathbb{N}$, there exists an interval $I = [\alpha_1,\alpha_2 ]\in \mathcal{I}_j$ such that $\mu_{h(\alpha_1)}\neq \mu_{h(\alpha_2)}$ and $\alpha^\star \in I$.\\\\
% %
% %
% We define $j' \in \mathbb{N}$ as the last iteration executed at Line~\dots; thus, $j' \in \mathbb{N}$ satisfies $\Delta_{j'} < \nicefrac{\gamma}{2}$.
% %
% Furthermore, let $I = [\alpha_1,\alpha_2 ]\in\mathcal{I}_{j’-1}$ be such that $\mu_{h(\alpha_1)}\neq \mu_{h(\alpha_2)}$ and $\alpha^\star \in I$. 
% %
% Notice that such interval exits thanks to Lemma~\dots.
% %
% Then:
% %
% \begin{enumerate}
% \item If $|I|\le \nicefrac{1}{T}$, then $I \in \mathcal{I}_{j’}$. This can be shown by following the analysis of point (2) in Lemma~\dots
% %
% \item If $|I|>\nicefrac{1}{T}$, we show that there is an $[\alpha_1',\alpha_2'] \in \mathcal{I}_{j’}$ s.t. $\mu_{h(\alpha_1')}\neq \mu_{h(\alpha_2')}$, $\alpha^\star \in I’$ and $|I'|\le\nicefrac{1}{T}$.
% \end{enumerate}
% %
% We prove point (2) above by induction.
% %
% Let $([\alpha_1,\alpha_2 ],j,k)$ be an input to Algorithm~2 for some $k\geq1$, with $\mu_{h(\alpha_1)}\neq \mu_{h(\alpha_2)}$ and $\alpha^\star \in [\alpha_1,\alpha_2 ]$, then either there exists an interval  $I’=[\alpha_1',\alpha_2']$ such that $(I',j,k+1)$ is given as input to Algorithm~2 with $\mu_{h(\alpha_1')}\neq \mu_{h(\alpha_2')}$ and $\alpha^\star \in [\alpha_1',\alpha_2']$ or $|I| \le \nicefrac{1}{T}$.
% %
% To prove this, it is enough to observe that if $\mu_{h(\alpha_1)} \neq \mu_{h(\alpha_2)}$ and the size of $I$ is larger than $\nicefrac{1}{T}$, then Algorithm~2 collects a number of samples proportional to $\nicefrac{1}{\Delta_j^2}$ from both the extremes of $I$. Under the event $\mathcal{E}$, we have:  
% \[
% \widehat{\mu}(\alpha_2) - \widehat{\mu}(\alpha_1) \geq \mu_{h(\alpha_2)} - \mu_{h(\alpha_1)} - \frac{\Delta_j}{2} \geq \gamma - \frac{\Delta_j}{2} \geq \frac{3\gamma}{4} > \frac{\gamma}{2} = \Delta_j.
% \]
% Thus, the condition at Lines~\dots in Algorithm~2 is verified, and Algorithm~2 is recursively invoked with two input intervals $I', I''$ such that $I' \cup I'' = I$, and thus either $\alpha^\star \in I'$ or $\alpha^\star \in I''$.
% %
% In contrast
% %

% Consequently, there exists an interval $I = [\alpha_1,\alpha_2 ] \in \mathcal{I}_{j’}$ such that $\mu_{h(\alpha_1)}\neq \mu_{h(\alpha_2)}$ and $\alpha^\star \in I$.
% %
% We observe that when the interval $I$ is selected during the execution of the for loop at Line~\dots, the value of $H$ at Line~\dots is either $-\infty$ or equal to $\widehat{\mu}(\overline\alpha)$ for some $\overline\alpha \le \alpha_1$, and thus $\mu_{h(\overline \alpha)} \le \mu_{h(\alpha_1)}< \mu_{h(\alpha_2)}$.
% %
% %This is because $\mu_{h(\alpha_1)} < \mu_{h(\alpha_2)}$ and thus $\mu_{h(\widebar\alpha)} < \mu_{h(\alpha_2)}$.
% %
% Therefore, under the event $\mathcal{E}$, we have:
% %
% \begin{equation*}
% 	\widehat{\mu}(\alpha_2) - \widehat{\mu}(\alpha_2') \leq \mu_{h(\alpha_2)} - \mu_{h(\alpha_2')} + \frac{\Delta_j}{2} < \frac{\gamma}{4}. 
% \end{equation*}
% %
% Thus, the condition at Line~\dots is satisfied and $\alpha_2$ is added to the set $\mathcal{W}$.
% \end{proof}

% \begin{restatable}{lemma}{.,,,..}
% 	Under the event $\mathcal{E}$, the cardinality of $|\mathcal{W}|\le n$.
% \end{restatable}
% \begin{proof}
% 	%
% 	In the following we focus on the case in which the $\textnormal{UCB-1}$ algorithm at Line~\ref{line:ucb1} is executed.
% 	% 
% 	This is without loss of generality since during the execution of the for loop at Line~\ref{lin:forLoopDep}, the size of $\mathcal{W}$ can only increase.
% 	%
% 	We define $j' \in \mathbb{N}_{+}$ as the smallest integer such that $\Delta_{j'} < \nicefrac{\gamma}{2}$.
% 	% 
% 	Intuitively, $j' \in \mathbb{N}_{+}$ corresponds to the largest epoch executed at Lines~....
	
% 	Let $i \in [n]$. We prove that, under the event $\mathcal{E}$, there exists at most a single $\alpha_2 \in \mathcal{W}$ such that $\mu_{h(\alpha_2)} = \mu_i$.
% 	% 
% 	Let $I \coloneqq [\alpha_1, \alpha_2]$ be an interval in $\mathcal{I}_{j'}$ such that, for any other distinct interval $I' \coloneqq [\alpha_1', \alpha_2']$ with $\mu_i = \mu_{h(\alpha_2')} = \mu_{h(\alpha_2)}$, it holds that $\alpha_2 < \alpha_2'$.
% 	% 
% 	We observe that, during the execution of the for loop at Line~\ref{lin:forLoopDep}, the interval $I$ is selected before any interval $I'$ satisfying the above relationship.
% 	% 
% 	This is because the intervals in $\mathcal{I}_{j}$ are sorted in increasing order, and the intersection between two consecutive intervals in $\mathcal{I}_{j}$ is either empty or a singleton.
	
% 	When $I$ is selected during the execution of the for loops at Line~\ref{lin:forLoopDep}, the value of $H$ is either $-\infty$ or equal to the empirical estimate $\widehat{\mu}(\overline \alpha)$ for some $\overline\alpha$, where $\mu_{h(\overline\alpha)} = \mu_{i'}$ with $i \neq i'$ due to the definition of $I$.
% 	% 
% 	Thus, under the event $\mathcal{E}$, we have:
% 	 \begin{equation*}
% 		\widehat{\mu}(\alpha_2) - H \geq \widehat{\mu}(\alpha_2) - \widehat{\mu}(\overline\alpha) \geq \mu_{h(\alpha_2)} - \mu_{h(\overline \alpha)} - \frac{\Delta_{j'}}{2} \geq \frac{3\gamma}{4}. 
% 		\end{equation*}
% 	% 
% 	Therefore, under the event $\mathcal{E}$, the condition at Line~\ref{line:IfElseDep} is true and the value of $H$ is updated to $\widehat{\mu}(\alpha_2')$.
	
% 	When any interval $I'$, defined as above, is selected during the execution of the for loops at Line~\ref{lin:forLoopDep}, we have:
% 	%
% 	\begin{equation*}
% 		\widehat{\mu}(\alpha_2) - \widehat{\mu}(\alpha_2') \leq \mu_{h(\alpha_2)} - \mu_{h(\alpha_2')} + \frac{\Delta_j}{2} < \frac{\gamma}{4}. 
% 	\end{equation*}
% 	%
% 	As a result, the value of $H$ remains unchanged because the condition at Line~ \ref{line:IfElseDep} is false, and $\alpha_2'$ is not added to $\mathcal{W}$.
% 	 %
% 	 Thus, for each $i \in [n]$, one of the following conditions holds:
% 	 %
% 	 \begin{enumerate}
% 	 	\item There is no interval $[\alpha_1,\alpha_2]\in \mathcal{I}_{j'}$ such that $\mu_{h(\alpha_2)}=\mu_i$.
% 	 	\item There is an interval $[\alpha_1,\alpha_2] \in \mathcal{I}_{j'}$ such that $\mu_{h(\alpha_2)}=\mu_i$.
% 	 	%
% 	 	Then, for each interval $[\alpha_1',\alpha_2']  \in \mathcal{I}_{j'}$ with $\alpha_2'>\alpha_2$ and $\mu_{h(\alpha_2)}=\mu_{h(\alpha_2')}$, it holds $\alpha_2'\not \in \mathcal{W}$.
% 	 \end{enumerate}
% 	 %
% 	 Therefore, for each $i \in [n]$, there is at most an $\alpha_2 \in \mathcal{W}$, concluding the proof.
% \end{proof}

% \begin{algorithm}[!htp]
% 	\caption{\texttt{Recursive Jump Identification with Optimistic Shrinking (RJI-OS)}}
% 	\label{alg:instance_dep}
% 	\begin{algorithmic}[1]
% 		\Require Number of rounds $T \in \mathbb{N}_+$, $\gamma$
% 		\State Set $\mathcal{I}_1 \gets \{ [0,1] \}$, $ \mathcal{T}_{1}\gets \{ \varnothing \}$ 
% 		\For{ $j \in \mathbb{N}_{+}$} 
% 		% State	$\Delta=2^{-j}$
% 		\If{$\Delta_j\ge \gamma/2$ }
% 		\State Execute Lines~\ref{line:endformain}-\ref{line:end_first_algo} in Algorithm~\ref{alg:main}
% 		\Else
% 		\State $H=-\infty$ and $\mathcal{W}=\varnothing$
% 		\For{ $[\alpha_1,\alpha_2] \in \mathcal{I}_j$} \label{lin:forLoopDep}
% 		\State Play $\alpha_2$ $\mathcal{O}( \nicefrac{1} {\Delta_j^2}\log(\nicefrac{1}{\delta}))$ times and set $\widehat \mu(\alpha_2)$ equal to the observed empirical mean
% 		\If{$\widehat \mu(\alpha_2)- H> 3/4 \gamma $} \label{line:IfElseDep}
% 		\State $H=\widehat \mu(\alpha_2)$ $\mathcal{W}=\mathcal{W}\cup \{\alpha_2\}$
% 		\EndIf
% 		\EndFor
% 		\State Run UCB-1 on the set $\mathcal{W}$ \label{line:ucb1}
% 		\EndIf
% 		\EndFor
% 	\end{algorithmic}
% \end{algorithm}
